Deterministic Document Exchange Protocols, and Almost Optimal Binary Codes for Edit Errors

We study two basic problems regarding edit error, i.e. document exchange and error correcting codes for edit errors (insdel codes). For message length $n$ and edit error upper bound $k$, it is known that in both problems the optimal sketch size or the optimal number of redundant bits is $\Theta(k \log \frac{n}{k})$. However, known constructions are far from achieving these bounds. We significantly improve previous results on both problems. For document exchange, we give an efficient deterministic protocol with sketch size $O(k\log^2 \frac{n}{k})$. This significantly improves the previous best known deterministic protocol, which has sketch size $O(k^2 + k \log^2 n)$ (Belazzougui15). For binary insdel codes, we obtain the following results: 1. An explicit binary insdel code which encodes an $n$-bit message $x$ against $k$ errors with redundancy $O(k \log^2 \frac{n}{k})$. In particular this implies an explicit family of binary insdel codes that can correct $\varepsilon$ fraction of insertions and deletions with rate $1-O(\varepsilon \log^2 (\frac{1}{\varepsilon}))=1-\widetilde{O}(\varepsilon)$. 2. An explicit binary insdel code which encodes an $n$-bit message $x$ against $k$ errors with redundancy $O(k \log n)$. This is the first explicit construction of binary insdel codes that has optimal redundancy for a wide range of error parameters $k$, and this brings our understanding of binary insdel codes much closer to that of standard binary error correcting codes. In obtaining our results we introduce the notion of \emph{$\varepsilon$-self matching hash functions} and \emph{$\varepsilon$-synchronization hash functions}. We believe our techniques can have further applications in the literature.

==> application.tex <==
\section{Applications}

\subsection{Insertion deletion codes}
Based on the result of the document exchange protocol, we can construct binary codes which is decodable from $k$ edit errors. The idea is that the information sent by Alice in the document exchange protocol can be regarded as a sketch with which we can reconstruct the original message. In this section we use $sk_m(n,k)$ to denote the message sent from Alice in an document exchange protocol where $n$ is the input size, $k$ is the upper bound of the edit distance and $m$ is the string hold by Alice.

\begin{theorem}
\label{codeFromSk}
If there exists a document exchange protocol with cost $|sk_m(k,n)|$ where $n$ is the input size and $k$ is the upper bound of edit distance, then there exists a code $C$ with encoding map: $Enc:\{0,1\}^n\mapsto\{0,1\}^{N}$ which can be decoded from $k$ insertion deletion errors. Here $N = n+O(|sk_m(3k,n)|)$.
\end{theorem}

\begin{proof}
The encoding algorithm is as follows: for message $m\in\{0,1\}^n$, we first compute the sketch $sk_m(3k,n)$ for $m$ from $3k$ insertion deletion errors. Then we encode the sketch $sk_m(3k,n)$ to be $\tilde{c}$ using the binary code in \cite{796406} constructed by Schulman and Zuckerman which can correct $\alpha$ fraction of errors with constant rate. Here $\alpha$ is a constant such that $\alpha|sk_m(sk,n)|\geq 3k$. This can be done because $|sk_m(sk,n)|$ contains a factor of $3k$. The final codeword $c$ is the concatenation of the original message $m$ and encoded sketch $\tilde{c}$. That is, $c=m\circ \tilde{c}$ and $|c| = N = n+ O(|sk_m(3k,n)|)$.

Now we show that this code can be decoded from $k$ edit errors. Denote the codeword after $k$ edit operations as $c'=m'\circ \tilde{c}'$ where $m'$ and $\tilde{c}'$ are the modified $m$ and $\tilde{c}$ respectively. Without loss of generality assume that $|c'|=N$. First we decode $c'(n+k,N]$ using the decoding algorithm of code in \cite{796406}. As there're only $k$ edit operations in total, the end of $m'$ must be in position from $n-k$ to $n+k$. This indicates that $ED(c'(n+k, N],\tilde{c}')\leq 2k$. Moreover, as $ED(\tilde{c}',\tilde{c})\leq k$, the edit distance between $c'(n+k, N]$ and $\tilde{c}$ is at most $3k$. Notice that $\tilde{c}$ can be decoded from $\alpha$ fraction of errors which are larger than $3k$, we can have the correct $sk_m(3k,n)$ after decoding $c'(n+k,N]$.


Then pick $\tilde{m}=c'[1,n-k]$. We have that $ED(\tilde{m},m)\leq 3k$ by similar argument as above. With $sk_m(3k,n)$ and $\tilde{m}$ we can correctly recover $m$.
\end{proof}


In \cite{7835185} Guruswarmi and Wang introduced binary insertion deletion codes that can correct $\eps$ fraction of edit errors with rate $1-\tilde{O}(\sqrt{\eps})$. According to Theorem \ref{codeFromSk}, we can construct a binary code for $\eps$ fraction of insertion deletion errors with rate $1-\tilde{O}(\eps)$, which is near optimal.


\begin{theorem}
\label{epsFracErr}
Let $\eps>0$ be a constant. There is a binary code $C$ with encoding map $Enc:\{0,1\}^n\mapsto\{0,1\}^{n+O(\eps n\log^2(1/\eps))}$ which can be decoded from $\eps n$ insertion deletion errors with rate $1-\tilde{O}(\eps)$.
\end{theorem}


\begin{proof}
To show this, we'll use the document exchange protocol in Construction \ref{dIMS}. Thus $|sk_m(3\eps n,n)|=O(\eps n\log^2(1/\eps))$. According to Theorem \ref{codeFromSk}, the code can be decoded from $\eps n$ edit errors. The rate $r$ of this code is thus $\frac{n}{n+O(\eps n\log^2(1/\eps))}= 1-\tilde{O}(\eps)$.
\end{proof}

%\begin{lemma}[Theorem IV.7 in \cite{7541373}]
%\label{constRateCode}
%Fix an integer $F\geq 2$ and $\alpha>0$. For infinitely many and sufficiently large $M$, there is an explicit code $C\subset\{0,1\}^M$ with rate $r(F,\alpha)=(\alpha/F)^{O(\alpha^{-12})}$ over a size $F$ alphabet that can be decoded from a $1-\frac{2}{F+1}-\alpha$ fraction of worst-case insertions and deletions in time $O_{F,\alpha}(M^3\poly\log(M))$. Furthermore, this code is constructible in time $O_{F,\alpha}(M\log^2M)$.
%\end{lemma}

Similarly for general $k$ edit errors, we can construct codes with document exchange protocol in Construction \ref{firststage}.

\begin{theorem}
\label{generalKError}
There exists a binary code $C$ with encoding map $Enc:\{0,1\}^n\mapsto\{0,1\}^{n+O(k\log n \log\log n)}$ which can be decoded from $k$ edit errors with $O(k\log n \log\log n)$ redundancy bits.
\end{theorem}

\begin{proof}
To show this, we'll use the document exchange protocol in Construction \ref{firststage}. Thus $|sk_m(3k,n)|=O(k\log n\log\log n)$. According to Theorem \ref{codeFromSk}, the code can be decoded from $k$ edit errors.
\end{proof}

If $k$ is a constant, then we have near-optimal redundancy bits.

